All-Hex Meshing Strategies For Densely Packed Spheres

We develop an all-hex meshing strategy for the interstitial space in beds of densely packed spheres that is tailored to turbulent flow simulations based on the spectral element method (SEM). The SEM achieves resolution through elevated polynomial order N and requires two to three orders of magnitude fewer elements than standard finite element approaches do. These reduced element counts place stringent requirements on mesh quality and conformity. Our meshing algorithm is based on a Voronoi decomposition of the sphere centers. Facets of the Voronoi cells are tessellated into quads that are swept to the sphere surface to generate a high-quality base mesh. Refinements to the algorithm include edge collapse to remove slivers, node insertion to balance resolution, localized refinement in the radial direction about each sphere, and mesh optimization. We demonstrate geometries with 10^2-10^5 spheres using approximately 300 elements per sphere (for three radial layers), along with mesh quality metrics, timings, flow simulations, and solver performance.

==> tex/mesh_table.tex <==
% MATLAB runs on
% HP Z840 Workstation, having 2 CPU sockets per node.
% Intel(R) Xeon(R) CPU E5-2630 v3 @ 2.40GHz
% Each CPU has 8 core / 16 threads.
% In total, it can run up to 16 cores / 32 threads.


%% Version 1 (before speed up)
%   \begin{table*}
%   \footnotesize
%   \begin{center}
%   \begin{tabular}{|l|r|r|r|r|r|r|r|}
%   \hline
%     \multicolumn{8}{|c|}{{\bf Meshing Time Breakdown (sec)}} \\
%     \hline
%   Meshing Procedure & cyl146 & cyl1568 & ann3344 & cyl11k & cyl49k & ann127k & ann350k \\
%                     &  N=2 &  N=2  &  N=2  &  N=2  &  N=2  & N=2 & N=7     \\
%   \hline
%   \hline
%   %Number of elements,$E$  
%   %        &      146 &     1568 &     3344 &    11145 &    49967 &   127602 &   353625\\ \hline
%   % Sphere Configurations
%   %       &Experiment& StarCCM+ & Project Chrono & Project Chrono & Project Chrono & StarCCM+ & StarCCM+\\
%   %        &Exp.& DEM1 & DEM2 & DEM2 & DEM2 & DEM1 & DEM1\\ \hline
%     IO for Qhull
%           & 4.56E-01 & 1.10E+00 & 2.64E+00 & 6.36E+00 & 1.97E+01 & 5.13E+01 & 2.79E+02\\
%   %      & Generate Qhull input 
%   %       & 2.51E-02 & 1.88E-02 & 4.63E-02 & 1.09E-01 & 2.63E-01 & 6.81E-01 & 2.62E+00\\
%     Voronoi cells (Qhull)
%           & 1.70E-01 & 4.29E-01 & 1.07E+00 & 2.50E+00 & 8.77E+00 & 2.12E+01 & 7.98E+01\\ 
%   %      & Read Qhull output 
%   %       & 4.31E-01 & 1.08E+00 & 2.60E+00 & 6.25E+00 & 1.95E+01 & 5.06E+01 & 2.77E+02\\ 
%   \hline
%   \hline
%     Facet generation
%           & 9.37E-01 & 6.79E+00 & 1.50E+01 & 5.71E+01 & 4.69E+02 & 3.41E+03 & 4.70E+04\\ 
%   %       & total 
%   %        & 2.39E+00 & 1.04E+01 & 2.14E+01 & 7.38E+01 & 5.33E+02 & 3.58E+03 & 4.81E+04\\
%     Edge collapse
%           & 8.67E-02 & 2.34E-01 & 4.53E-01 & 1.26E+00 & 5.24E+00 & 1.30E+01 & 8.20E+01\\
%     Facet/edge clean-up 
%           & 1.21E+00 & 6.57E+00 & 8.66E+00 & 2.75E+01 & 1.29E+02 & 3.47E+02 & 2.55E+03\\
%   \hline
%   \hline
%     Tessellation 
%           & 2.37E+00 & 1.40E+01 & 2.78E+01 & 9.62E+01 & 7.30E+02 & 4.09E+03 & 2.62E+04\\ 
%     All-quad generation
%           & 1.67E-01 & 7.02E-01 & 1.34E+00 & 4.24E+00 & 1.74E+01 & 4.61E+01 & 1.20E+02\\ 
%   %       & total 
%   %        & 4.35E+00 & 2.62E+01 & 5.20E+01 & 1.72E+02 & 1.05E+03 & 4.97E+03 & 2.85E+04\\
%   \hline
%   \hline
%     All-quad to all-hex 
%           & 5.64E-02 & 2.48E-01 & 5.13E-01 & 2.42E+00 & 9.34E+00 & 2.52E+01 & 7.97E+01\\
%     Extrusion 1
%           & 4.99E-01 & 3.58E+00 & 8.60E+00 & 2.11E+01 & 8.58E+01 & 3.10E+02 & 1.63E+03\\ 
%   %       & total 
%   %        & 2.10E+00 & 1.09E+01 & 2.13E+01 & 6.34E+01 & 2.74E+02 & 7.46E+02 & 3.17E+03\\
%   \hline
%   \hline
%    IO for smoothing 
%           & 2.42e-01 & 4.99E+00 & 4.13E+00 & 1.30E+01 & 5.85E+01 & 1.96E+02 & 1.12E+03\\ 
%    Mesh smoothing 
%           & 3.58e+00 & 4.12E+01 & 9.95E+01 & 3.99E+02 & 7.26E+02 & 3.19E+03 & 1.10E+03\\ 
%    (nodes)& (1)      &(1)       &  (1)     &    (2)   &   (4)    & (8)      &   (24)  \\
%   %       &(42 cores)&(42 cores)&(42 cores)&(84 cores)&(168 cores)&(336 cores)&(1008 cores)\\
%   %       & total 
%   %        & 3.82E+00 & 4.62E+01 & 1.04E+02 & 4.12E+02 & 7.85E+02 & 3.38E+03 & 2.22E+03\\
%   \hline
%   \hline
%     Extrusion 2
%           & 1.01E+00 & 5.36E+00 & 1.08E+01 & 2.80E+01 & 1.10E+02 & 6.72E+02 & 2.12E+03\\
%   \hline
%   \hline
%     IO for projection
%   %      & dump dat 
%   %      & 9.56E-03 & 4.59E-02 & 9.95E-02 & 2.57E-01 & 1.34E+00 & 7.23E+00 & 1.88E+01 \\
%   %      &&   6.8 KB &  71.4 KB & 152.1 KB & 506.3 KB &   2.2 MB &   5.7 MB &  15.6 MB\\
%   %      & dump co2 
%   %      & 2.86E-02 & 1.27E-01 & 2.45E-01 & 7.64E-01 & 3.40E+00 & 1.27E+02 & 7.11E+01 \\
%   %      &&   2.2 MB &  18.2 MB &  37.1 MB & 117.0 MB & 476.9 MB &   1.2 GB &   3.3 GB\\
%   %      & dump re2 
%   %      & 1.17E-01 & 5.98E-01 & 1.27E+00 & 4.11E+00 & 1.72E+01 & 2.70E+01 & 3.26E+02 \\
%   %      &&  14.7 MB & 123.3 MB & 250.2 MB & 787.3 MB &   3.1 GB &   8.4 GB &  22.3 GB\\
%   %      & total 
%          & 1.55E-01 & 7.71E-01 & 1.62E+00 & 5.13E+00 & 2.19E+01 & 1.62E+02 & 4.16E+02 \\
%     Curve-side projection 
%          & 4.00E+01 & 2.10E+02 & 1.80E+03 & 1.68E+03 & 4.20E+03 & 3.60E+03 & 7.20E+03 \\
%   (nodes)& (1)      &(1)       &  (1)     &    (2)   &   (4)    & (8)      &   (600)  \\
%   %      &(42 cores)&(42 cores)&(42 cores)&(84 cores)&(168 cores)&(336 cores)&(25200 cores)\\
%   \hline
%   \hline
%    Total  & 6.71E+01 & 3.41E+02 & 2.05E+03 & 2.55E+03 & 7.51E+03 & 1.89E+04 & 1.88E+05\\
%   \hline
%   \end{tabular}
%   \end{center}
%   \caption{\label{tb:meshtime}
%   %Breakdown of meshing times (seconds, unless otherwise indicated).  Most
%   Timing breakdown of meshing measured in seconds.
%   Most procedures are performed in serial using Matlab on
%   a workstation (Intel Xeon E5-2630 v3 @2.40GHz) while the ones performed in parallel 
%   are provided with the number of nodes. 
%   The smoothing and projection are performed on OLCF/Summit using 42 cores per node. 
%   Note that the case of ann350k required the edge collapse twice with tolerance adjustment.}
%   \end{table*}





%% Version 2 (05/26 speed up tessellaion and facet generation)
\begin{table*}
\footnotesize
\begin{center}
\begin{tabular}{|l|r|r|r|r|r|r|r|}
\hline
  \multicolumn{8}{|c|}{{\bf Meshing Time Breakdown (sec)}} \\
  \hline
Meshing Step & cyl146 & cyl1568 & ann3344 & cyl11k & cyl49k & ann127k & ann350k \\
%                 &  N=2 &  N=2  &  N=2  &  N=2  &  N=2  & N=2 & N=7     \\
\hline
\hline
%Number of elements,$E$  
%        &      146 &     1568 &     3344 &    11145 &    49967 &   127602 &   353625\\ \hline
% Sphere Configurations
%       &Experiment& StarCCM+ & Project Chrono & Project Chrono & Project Chrono & StarCCM+ & StarCCM+\\
%        &Exp.& DEM1 & DEM2 & DEM2 & DEM2 & DEM1 & DEM1\\ \hline
  IO for Qhull
        & 4.56E-01 & 1.10E+00 & 2.64E+00 & 6.36E+00 & 1.97E+01 & 5.13E+01 & 2.79E+02\\
%      & Generate Qhull input 
%       & 2.51E-02 & 1.88E-02 & 4.63E-02 & 1.09E-01 & 2.63E-01 & 6.81E-01 & 2.62E+00\\
  Voronoi cells (Qhull)
        & 1.70E-01 & 4.29E-01 & 1.07E+00 & 2.50E+00 & 8.77E+00 & 2.12E+01 & 7.98E+01\\ 
%      & Read Qhull output 
%       & 4.31E-01 & 1.08E+00 & 2.60E+00 & 6.25E+00 & 1.95E+01 & 5.06E+01 & 2.77E+02\\ 
\hline
\hline
  Facet generation
        & 1.66E-01 & 1.51R+00 & 4.22E+00 & 1.90E+01 & 1.77E+02 & 9.14E+02 & 4.20E+03\\ %new
%       & total 
%        & 8.07E-01 & 4.65E+00 & 1.08E+01 & 4.02E+01 & 2.65E+02 & 1.10E+03 & 4.66E+03\\%new

  Edge collapse
        & 8.67E-02 & 2.34E-01 & 4.53E-01 & 1.26E+00 & 5.24E+00 & 1.30E+01 & 8.20E+01\\
  Facet/edge clean-up 
        & 1.21E+00 & 6.57E+00 & 8.66E+00 & 2.75E+01 & 1.29E+02 & 3.47E+02 & 2.55E+03\\
\hline
\hline
  Tessellation 
        & 1.43E+00 & 9.76E+00 & 1.87E+01 & 6.26E+01 & 2.84E+02 & 6.70E+02 & 1.65E+03\\% new

  All-quad generation
        & 1.67E-01 & 7.02E-01 & 1.34E+00 & 4.24E+00 & 1.74E+01 & 4.61E+01 & 1.20E+02\\ 
%       & total 
%        & 4.35E+00 & 2.62E+01 & 5.20E+01 & 1.72E+02 & 1.05E+03 & 4.97E+03 & 2.85E+04\\
\hline
\hline
  All-quad to all-hex 
        & 5.64E-02 & 2.48E-01 & 5.13E-01 & 2.42E+00 & 9.34E+00 & 2.52E+01 & 7.97E+01\\
  Extrusion 1
        & 4.99E-01 & 3.58E+00 & 8.60E+00 & 2.11E+01 & 8.58E+01 & 3.10E+02 & 1.63E+03\\ 
%       & total 
%        & 2.10E+00 & 1.09E+01 & 2.13E+01 & 6.34E+01 & 2.74E+02 & 7.46E+02 & 3.17E+03\\
\hline
\hline
  IO for smoothing 
        & 2.42e-01 & 4.99E+00 & 4.13E+00 & 1.30E+01 & 5.85E+01 & 1.96E+02 & 1.12E+03\\ 
  Mesh smoothing 
        & 3.58e+00 & 4.12E+01 & 9.95E+01 & 3.99E+02 & 7.26E+02 & 3.19E+03 & 1.10E+03\\ 
  (nodes, $N$)
        &  (1, $N$=1) &(1, $N$=1) &(1, $N$=1) &(2, $N$=1) &(4, $N$=1) &(8, $N$=1) &(24, $N$=1)\\%update
%       &(42 cores)&(42 cores)&(42 cores)&(84 cores)&(168 cores)&(336 cores)&(1008 cores)\\
%       & total 
%        & 3.82E+00 & 4.62E+01 & 1.04E+02 & 4.12E+02 & 7.85E+02 & 3.38E+03 & 2.22E+03\\
\hline
\hline
  Extrusion 2
        & 1.01E+00 & 5.36E+00 & 1.08E+01 & 2.80E+01 & 1.10E+02 & 6.72E+02 & 2.12E+03\\
\hline
\hline
  IO for projection
%      & dump dat 
%      & 9.56E-03 & 4.59E-02 & 9.95E-02 & 2.57E-01 & 1.34E+00 & 7.23E+00 & 1.88E+01 \\
%      &&   6.8 KB &  71.4 KB & 152.1 KB & 506.3 KB &   2.2 MB &   5.7 MB &  15.6 MB\\
%      & dump co2 
%      & 2.86E-02 & 1.27E-01 & 2.45E-01 & 7.64E-01 & 3.40E+00 & 1.27E+02 & 7.11E+01 \\
%      &&   2.2 MB &  18.2 MB &  37.1 MB & 117.0 MB & 476.9 MB &   1.2 GB &   3.3 GB\\
%      & dump re2 
%      & 1.17E-01 & 5.98E-01 & 1.27E+00 & 4.11E+00 & 1.72E+01 & 2.70E+01 & 3.26E+02 \\
%      &&  14.7 MB & 123.3 MB & 250.2 MB & 787.3 MB &   3.1 GB &   8.4 GB &  22.3 GB\\
%      & total 
       & 1.55E-01 & 7.71E-01 & 1.62E+00 & 5.13E+00 & 2.19E+01 & 1.62E+02 & 4.16E+02 \\
  Curve-side projection 
       & 4.00E+01 & 2.10E+02 & 1.80E+03 & 1.68E+03 & 4.20E+03 & 3.60E+03 & 7.20E+03 \\
  (nodes, $N$)
       & (1, $N$=2) &(1, $N$=2) &(1, $N$=2) &(2, $N$=2) &(4, $N$=2) &(8, $N$=2) &(600, $N$=7) \\%update
%      &(42 cores)&(42 cores)&(42 cores)&(84 cores)&(168 cores)&(336 cores)&(25200 cores)\\
\hline
\hline
%Total  & 6.71E+01 & 3.41E+02 & 2.05E+03 & 2.55E+03 & 7.51E+03 & 1.89E+04 & 1.88E+05\\% old
 Total  & 6.53E+01 & 2.70E+02 & 1.91E+03 & 2.04E+03 & 4.27E+03 & 1.09E+03 & 5.10E+04\\% new

\hline
\end{tabular}
\end{center}
\caption{\label{tb:meshtime}
Timing breakdown of meshing measured in seconds.  Most steps are performed in
serial using Matlab on a workstation (Intel Xeon E5-2630 v3 @2.40GHz) while the
ones performed in parallel are provided with the number of nodes and the
polynomial order $N$.  The smoothing and projection are performed on
OLCF/Summit using 42 cores per node.  Note that the case of ann350k required
two passes through the entire procedure to adjust the edge-collapse tolerance.
}
\end{table*}

